Exploring the Maze of Multilingual Modeling

Multilingual language models have gained significant attention in recent years, enabling the development of applications that meet diverse linguistic contexts. In this paper, we present a comprehensive evaluation of three popular multilingual language models: mBERT, XLM-R, and GPT-3. We assess their performance across a diverse set of languages, with a focus on understanding the impact of resource availability (general and model-specific), language family, script type, and word order on model performance, under two distinct tasks - text classification and text generation. Our findings reveal that while the amount of language-specific pretraining data plays a crucial role in model performance, we also identify other factors such as general resource availability, language family, and script type, as important features. We hope that our study contributes to a deeper understanding of multilingual language models to enhance their performance across languages and linguistic contexts.

==> wordorder.tex <==
\subsection{Impact of Word order}

Word order, also known as linear order, refers to the arrangement of syntactic constituents within a language. The study of word order typology examines how different languages employ distinct orders. In Figure \ref{figure:word-order}, we present the accuracy of different models across three word orders. Notably, we observe that word order has a relatively minor impact on the accuracy of \texttt{mBERT} and \texttt{XLM-R}, whereas it significantly affects the performance of \texttt{GPT-3}.

\texttt{GPT-3} demonstrates better accuracy on subject-verb-object (SVO) languages compared to subject-object-verb (SOV) languages across all resource levels. Additionally, \texttt{GPT-3} achieves its best performance on verb-subject-object (VSO) languages, even though they are classified as low resource languages. These findings indicate that word order plays a significant role in shaping the performance of \texttt{GPT-3}, suggesting a heightened sensitivity of the model to the structural characteristics of different word orders.


\begin{figure*}[ht]
\centering
\includegraphics[width=0.7\textwidth]{Figs/word-order.png}
\caption{Average accuracy of \texttt{GPT-3}, \texttt{XLM-R}, and \texttt{mBERT} by word order, broken down by resources.}
\label{figure:word-order}
\end{figure*}
